Transfer Learning with Large-Scale Quantile Regression

Quantile regression is increasingly encountered in modern big data applications due to its robustness and flexibility. We consider the scenario of learning the conditional quantiles of a specific target population when the available data may go beyond the target and be supplemented from other sources that possibly share similarities with the target. A crucial question is how to properly distinguish and utilize useful information from other sources to improve the quantile estimation and inference at the target. We develop transfer learning methods for high-dimensional quantile regression by detecting informative sources whose models are similar to the target and utilizing them to improve the target model. We show that under reasonable conditions, the detection of the informative sources based on sample splitting is consistent. Compared to the naive estimator with only the target data, the transfer learning estimator achieves a much lower error rate as a function of the sample sizes, the signal-to-noise ratios, and the similarity measures among the target and the source models. Extensive simulation studies demonstrate the superiority of our proposed approach. We apply our methods to tackle the problem of detecting hard-landing risk for flight safety and show the benefits and insights gained from transfer learning of three different types of airplanes: Boeing 737, Airbus A320, and Airbus A380.

==> Makefile <==
source := $(wildcard tlqr.tex)
bib := $(wildcard *.bib)
out := $(patsubst %.tex,%.pdf,$(source))
latest := $(shell git log -1 --pretty=format:"%h")
rev := $(latest)

.PHONY: all
all: $(out)

%.pdf: %.tex $(bib)
	@latexmk -halt-on-error -pdf $<
##	@latexmk -c

## compare modification with the latest version checked into git
## for comparison of specific commits:
##	latexdiff-vc --git -r old_githash -r new_githash --pdf source.tex
diff:
	latexdiff-vc --git --pdf --force $(source) -r $(rev)

log:
	@git log -5 --pretty=format:"%h by %an at %ar: %s" $(source)

.PNONY: clean
clean:
	rm -rf $(out) *~ .*~ .\#* .Rhistory *.aux *.bbl *.blg *.dvi *.out *.log *.toc \
	*.fff *.fdb_latexmk *.fls *.ttt *diff* *oldtmp* .blb

